Compact Binary Waveform Center-of-Mass Corrections

We present a detailed study of the center-of-mass (c.m.) motion seen in simulations produced by the Simulating eXtreme Spacetimes (SXS) collaboration. We investigate potential physical sources for the large c.m. motion in binary black hole simulations and find that a significant fraction of the c.m. motion cannot be explained physically, thus concluding that it is largely a gauge effect. These large c.m. displacements cause mode mixing in the gravitational waveform, most easily recognized as amplitude oscillations caused by the dominant (2,$\pm$2) modes mixing into subdominant modes. This mixing does not diminish with increasing distance from the source; it is present even in asymptotic waveforms, regardless of the method of data extraction. We describe the current c.m.-correction method used by the SXS collaboration, which is based on counteracting the motion of the c.m. as measured by the trajectories of the apparent horizons in the simulations, and investigate potential methods to improve that correction to the waveform. We also present a complementary method for computing an optimal c.m. correction or evaluating any other c.m. transformation based solely on the asymptotic waveform data.

==> Affiliations.tex <==
%auto-ignore

\newcommand{\Caltech}{\affiliation{Theoretical Astrophysics, Walter
    Burke Institute for Theoretical Physics, MC 350-17, California
    Institute of Technology, Pasadena, California 91125, USA}} %

\newcommand{\Cornell}{\affiliation{Cornell Center for Astrophysics and
    Planetary Science, Cornell University, Ithaca, New York 14853,
    USA}} %

\newcommand{\CITA}{\affiliation{Canadian Institute for Theoretical
    Astrophysics, University of Toronto, 60 Saint George Street,
    Toronto, Ontario M5S 3H8, Canada}} %

\newcommand{\AEI}{\affiliation{Albert-Einstein-Institut,
    Max-Planck-Institut f{\"{u}}r Gravitationsphysik, D-14476
    Potsdam-Golm, Germany}} %


==> Macros.tex <==
%auto-ignore


%%%%%%%%%%%%%%%%
%% Math forms %%
%%%%%%%%%%%%%%%%
\let\Originalddefinition\d
\renewcommand{\d}{\ensuremath{\mathrm{d}}}
\let\Originaledefinition\e
\newcommand{\e}{\ensuremath{\mathrm{e}}}
\let\Originalidefinition\i
\renewcommand{\i}{\ensuremath{\mathrm{i}}}
\DeclareSymbolFont{wasy}{U}{wasy}{m}{n}
\DeclareMathSymbol{\thorn}{\mathord}{wasy}{105}
\DeclareMathSymbol{\Thorn}{\mathord}{wasy}{106}
\newcommand\Eth{\text{\DH}}
\newcommand\Alpha{\mathrm{A}}
\newcommand\Beta{\mathrm{B}}
\newcommand\Epsilon{\mathrm{E}}
\newcommand\Varepsilon{\mathit{E}}
\newcommand\Zeta{\mathrm{Z}}
\newcommand\Eta{\mathrm{H}}
\newcommand\Vartheta{\varTheta}
\newcommand\Iota{\mathrm{I}}
\newcommand\Kappa{\mathrm{K}}
\newcommand\Mu{\mathrm{M}}
\newcommand\Nu{\mathrm{N}}
\chardef\omicron=111 % For insurance against upcasing
\chardef\Omicron=79  % For insurance against downcasing
\newcommand{\Varpi}{\varPi}
\newcommand\Rho{\mathrm{P}}
\newcommand\Varrho{\mathit{P}}
\newcommand\Varsigma{\varSigma}
\newcommand\Varphi{\varPhi}
\newcommand\Tau{\mathrm{T}}
\newcommand\Chi{\mathrm{X}}
\newcommand\MakeAllUppercase[1]{%
  % Include eth, thorn, and Greek in MakeUppercase
  \begingroup
  \let\eth\Eth
  \let\thorn\Thorn
  \let\alpha\Alpha
  \let\beta\Beta
  \let\gamma\Gamma
  \let\delta\Delta
  \let\epsilon\Epsilon
  \let\varepsilon\Varepsilon
  \let\zeta\Zeta
  \let\eta\Eta
  \let\theta\Theta
  \let\vartheta\Vartheta
  \let\iota\Iota
  \let\kappa\Kappa
  \let\lambda\Lambda
  \let\mu\Mu
  \let\nu\Nu
  \let\xi\Xi
  \let\omicron\Omicron
  \let\pi\Pi
  \let\varpi\Varpi
  \let\rho\Rho
  \let\varrho\Varrho
  \let\sigma\Sigma
  \let\varsigma\Varsigma
  \let\tau\Tau
  \let\upsilon\Upsilon
  \let\phi\Phi
  \let\varphi\Varphi
  \let\chi\Chi
  \let\psi\Psi
  \let\omega\Omega
  \MakeUppercase{#1}%
  \endgroup
}


%% Units
\let\Originalcdefinition\c
\renewcommand{\c}{\mathrm{c}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\MSun}{\ensuremath{M_\odot}\xspace}
\newcommand{\Sun}{\MSun}
\newcommand{\Mtot}{\ensuremath{M_\text{tot}}}
\DeclareSIUnit{\strain}{strain}
\DeclareSIPrePower{\root}{1/2}
\DeclareSIUnit{\parsec}{pc}
\DeclareSIUnit{\yr}{yr}
\DeclareSIUnit{\year}{yr}
\DeclareSIUnit{\lightyear}{ly}
\DeclareSIUnit{\SolarMass}{\ensuremath{\MSun}}
\DeclareSIUnit{\Mass}{\ensuremath{M}}
% \newcommand{\strain}{\text{strain}}
% \newcommand{\parsec}{\text{pc}}
% \newcommand{\SolarMass}{\MSun}

%% abs, norm, ceil, floor, avg, etc.
\newcommand{\abs} [1]{\left\lvert{#1}\right\rvert}
\newcommand{\norm}[1]{\left\lVert{#1}\right\rVert}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\avg}[1]{\left\langle{#1}\right\rangle}
\newcommand{\co}[1]{\ensuremath{\bar{#1}}}
\DeclareMathOperator*{\RS}{RiemannSymmetrize}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator{\arcsin}{arcsin}
% \DeclareMathOperator{\arccos}{arccos}
% \DeclareMathOperator{\arctan}{arctan}
\DeclareMathOperator{\arccsc}{arccsc}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\asinh}{arsinh}
\DeclareMathOperator{\acosh}{arcosh}
\DeclareMathOperator{\atanh}{artanh}
\DeclareMathOperator{\acsch}{arcsch}
\DeclareMathOperator{\asech}{arsech}
\DeclareMathOperator{\acoth}{arcoth}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\arcsch}{arcsch}
\DeclareMathOperator{\arsech}{arsech}
\DeclareMathOperator{\arcoth}{arcoth}

%% Relational operators
\newcommand{\defined}{\coloneqq}
\newcommand{\identically}{\equiv}
\newcommand{\roughly}{\mathord{\sim}} % Different from \sim in spacing
%\newcommand{\corresponds}{\triangleq}
\newcommand{\asymptoticallyequal}{\simeq}
\newcommand{\homeomorphic}{\cong}
\newcommand{\isomorphic}{\approx}



%% Asymptotically flat limits
\newcommand{\scri}{\ensuremath{\mathscr{I}}}
\newcommand{\scriplus}{\ensuremath{\mathscr{I}^{+}}}
\newcommand{\scriminus}{\ensuremath{\mathscr{I}^{-}}}
\newcommand{\Mirr}{\ensuremath{M_{\text{irr}}}}
\newcommand{\Eadm}{\ensuremath{M_{\text{ADM}}}}
\newcommand{\Jadm}{\ensuremath{J_{\text{ADM}}}}
\newcommand{\ADMMass}{\Eadm}
\newcommand{\IrrMass}{\Mirr}
\newcommand{\tr}{\ensuremath{t_\text{ret}}}
\newcommand{\rt}{\ensuremath{r_{\ast}}}

%% Wigner matrices, rotations, etc.
\newcommand{\trivialgroup}{\langle 0 \rangle}
\newcommand{\D}{\ensuremath{\mathfrak{D}} }
\newcommand{\R}{\ensuremath{\mathcal{R}} }
\newcommand{\threej}[6]{
  \begin{pmatrix}
    #1 & #2 & #3 \\ #4 & #5 & #6
  \end{pmatrix}
}
% \newcommand{\sYlm}[1]{\ensuremath{\prescript{}{s}{Y}_{#1}}}
% \newcommand{\mTwoYlm}[1]{\ensuremath{\prescript{}{-2}{Y}_{#1}}}
\newcommand{\sYlm}[1]{\ensuremath{\scripts{_{s}}{Y}{_{#1}}}}
\newcommand{\sYbarlm}[1]{\ensuremath{\scripts{_{s}}{\bar{Y}}{_{#1}}}}
\newcommand{\mTwoYlm}[1]{\ensuremath{\scripts{_{-2}}{Y}{_{#1}}}}
\newcommand{\mTwoYbarlm}[1]{\ensuremath{\scripts{_{-2}}{\bar{Y}}{_{#1}}}}
%\newcommand{\Rotated}[1]{\ensuremath{\accentset{\frown}{#1}}}
%\newcommand{\Rotated}[1]{\ensuremath{\breve{#1}}}
%\newcommand{\Rotated}[1]{\ensuremath{#1'}}
\DeclareSymbolFont{tipa}{T3}{tipa}{m}{n}
\DeclareMathAccent{\ibreve}{\mathalpha}{tipa}{'020}
\newcommand{\Rotated}[1]{\ensuremath{\ibreve{#1}}}
\newcommand{\Rotation}[1]{\mathbf{\MakeUppercase{#1}}}
\newcommand{\LieElement}[1]{\mathbf{\MakeUppercase{#1}}}
\newcommand{\LieComponent}[2]{\mathrm{\MakeUppercase{#1}}_{#2}}
\newcommand{\LieGenerator}[1]{\mathbf{\MakeLowercase{#1}}}
\newcommand{\LieGeneratorMag}[1]{\mathrm{\MakeLowercase{#1}}}
\newcommand{\GeneratorVec}[1]{\ensuremath{\vec{\MakeLowercase{#1}}}}
\DeclareMathOperator{\adjoint}{ad}
\DeclareMathOperator{\Adjoint}{Ad}
\newcommand{\ad}[1]{\adjoint_{\LieGenerator{#1}}}
\newcommand{\Ad}[1]{\Adjoint_{\LieGenerator{#1}}}
\newcommandx{\structure}[3][2={}, 3={}]{f^{#1 #2}_{#3}}
\newcommand{\RP}[1]{\mathbb{R}\mathrm{P}^{#1}}
\newcommand{\CP}[1]{\mathbb{C}\mathrm{P}^{#1}}

\newcommand{\SO}[1]{\ensuremath{\mathrm{SO}(#1)}}
%\newcommand{\so}[1]{\ensuremath{\mathfrak{so}(#1)}}
\newcommand{\SOp}[1]{\ensuremath{\mathrm{SO}^{+}(#1)}}
\newcommand{\sop}[1]{\ensuremath{\mathfrak{so}^{+}(#1)}}
\newcommand{\U}[1]{\ensuremath{\mathrm{U}(#1)}}
% \newcommand{\u}[1]{\ensuremath{\mathfrak{u}(#1)}}
\newcommand{\SU}[1]{\ensuremath{\mathrm{SU}(#1)}}
\newcommand{\su}[1]{\ensuremath{\mathfrak{su}(#1)}}
\newcommand{\SL}[1]{\ensuremath{\mathrm{SL}(#1)}}
\newcommand{\PSL}[1]{\ensuremath{\mathrm{PSL}(#1)}}
\newcommand{\Spin}[1]{\ensuremath{\mathrm{Spin}(#1)}}
\newcommand{\Spinplus}[1]{\ensuremath{\mathrm{Spin}^{+}(#1)}}
\newcommand{\spin}[1]{\ensuremath{\mathfrak{so}(#1)}}
\newcommand{\bms}{\ensuremath{\mathfrak{bms}}}

\newcommand{\HopfMap}{\mathfrak{h}}
\newcommand{\TangentBundle}[1]{\mathrm{T}\left(#1\right)}
\newcommand{\UnitTangentBundle}[1]{\mathrm{UT}\left(#1\right)}
\newcommand{\TangentBundleAt}[2]{\mathrm{T}_{#1}\left(#2\right)}
\newcommand{\UnitTangentBundleAt}[2]{\mathrm{UT}_{#1}\left(#2\right)}

%% Metric perturbation
\newcommand{\Background}[1]{\underaccent{\frown}{#1}}
\newcommand{\h}{\ensuremath{h} }
\newcommand{\hp}{\ensuremath{h_{+}} }
\newcommand{\hc}{\ensuremath{h_{\times}} }
\newcommand{\htilde}{\ensuremath{{\tilde{h}}}}
\newcommand{\Schw}{\ensuremath{\Background{R}} }
\newcommand{\GW}{\tilde{R}}
\newcommand{\Schwg}{\ensuremath{\Background{g}} }
\newcommand{\GWg}{\tilde{g}}
\newcommand{\SchwScalar}{\ensuremath{{\Background{\boxdot}}} }

%% Frequencies, discretization, DA stuff...
\newcommand{\fsamp}{\ensuremath{f_{\mathrm{s}}}}
\newcommand{\fNy}{\ensuremath{f_{\mathrm{Ny}}}}
\newcommand{\discretize}{\rightsquigarrow}
%%\newcommand{\MM}{\text{MM}} %% See below
\newcommand{\parameters}{\vec{\lambda}}
\newcommand{\response}{\ensuremath{\mathcal{R}}}
\newcommand{\phifid}{\ensuremath{\phi_{\text{fid}}}}
\newcommand{\ffid}{\ensuremath{f_{\text{fid}}}}
\newcommand{\tfid}{\ensuremath{t_{\text{fid}}}}
\newcommand{\tf}{\ensuremath{t_{(f)}}}
\newcommand{\tfOne}{\ensuremath{t_{1,(f)}}}
\newcommand{\tfTwo}{\ensuremath{t_{2,(f)}}}
\newcommand{\omegah}{\ensuremath{\omega_{\text{hyb}}}}
\newcommand{\fhyb}{\ensuremath{f_{\text{hyb}}}}
\newcommand{\thyb}{\ensuremath{t_{\text{hyb}}}}

%% Boldface (indexless) four-tensor notation
\newcommand{\Tensor}[1]{\bm{\mathsf{#1}}}
\newcommand{\FourVector}[1]{\bm{#1}}
\newcommand{\Vector}[1]{\FourVector{#1}}

%% Three-vector
\newcommand{\ThreeVector}[1]{\Vector{#1}}

\newcommand{\fourvec}[1]{\FourVector{#1}}
% \renewcommand{\threevec}[1]{\ensuremath{\vec{#1}}}
% \newcommand{\threevec}{\fourvec}
% \newcommand{\unitvec}[1]{\hat{\fourvec{#1}}}
\newcommand{\threevec}{\Vector}
\newcommand{\rHat}{\unitvec{r}}
\newcommand{\nHat}{\unitvec{n}}
\newcommand{\xHat}{\unitvec{x}}
\newcommand{\yHat}{\unitvec{y}}
\newcommand{\zHat}{\unitvec{z}}

\newcommand{\rapidity}{\varphi}

%% Polarization tensors
\newcommand{\pol}{\ensuremath{\varepsilon}}
\newcommand{\polp}{{\ensuremath{\pol_{+}}}}
\newcommand{\polc}{{\ensuremath{\pol_{\times}}}}

%% Transverse, traceless part
\newcommand{\TT}{\mathrm{TT}}


%%%%%%%%%%%%%%%%
%% Text forms %%
%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\foreign}[1]{\textit{#1}} % {\textrm{#1}}
\newcommand{\etal}{\foreign{et~al}\@ifnextchar{\relax}{.\relax}{\ifx\@let@token.\else\ifx\@let@token~.\else.\@\xspace\fi\fi}}
\newcommand{\etc}{\foreign{etc}\@ifnextchar{\relax}{.\relax}{\ifx\@let@token.\else\ifx\@let@token~.\else.\@\xspace\fi\fi}}
\newcommand{\eg}{\foreign{e.g}\@ifnextchar{\relax}{.\relax}{\ifx\@let@token.\else\ifx\@let@token~.\else.\@\xspace\fi\fi}}
\newcommand{\ie}{\foreign{i.e}\@ifnextchar{\relax}{.\relax}{\ifx\@let@token.\else\ifx\@let@token~.\else.\@\xspace\fi\fi}}
\newcommand{\perse}{\foreign{per~se}\xspace}
\newcommand{\cf}{\foreign{cf}\@ifnextchar{\relax}{.\relax}{\ifx\@let@token.\else\ifx\@let@token~.\else.\@\xspace\fi\fi}}
\makeatother

\newcommand{\pN}{\text{PN}\xspace}
\newcommand{\PN}{\pN\xspace}
\newcommand{\Pade}{{Pad{\'{e}}}\xspace}
\newcommand{\Poincare}{Poincar{\'{e}}\xspace}
\newcommand{\Bezier}{B{\'{e}}zier\xspace}
\newcommand{\Mobius}{M{\"{o}}bius\xspace}

\definecolor{NoteColor}{rgb}{0.900, 0.218, 0.000}
\newcommand{\Note}[1]{\textcolor{NoteColor}{[#1]}\index{Note}}
\definecolor{NoteQuietColor}{rgb}{0.300, 0.073, 0.000}
\newcommand{\NoteQuiet}[1]{\textcolor{NoteQuietColor}{[#1]}\index{NoteQuiet}}
\definecolor{NewColor}{rgb}{0,.55,0}
\newcommand{\New}[1]{\textcolor{NewColor}{#1}\index{New}}

\newcommand{\software}[1]{\texttt{#1}}
\newcommand{\command}[1]{\texttt{\small{#1}}}
\newcommand{\code}[1]{\texttt{\small{#1}}}


%%%%%%%%%%%%%%
%% Commands %%
%%%%%%%%%%%%%%
\makeatletter
%% For caption names
\newcommand{\CapName}[1]{\textbf{#1}.}
%% The following command allows you to enter \ShowDimensions anywhere
%% in a document, and -- at processing -- see all the dimensions (I
%% could think of) in the terminal.

\newcommand{\ShowDimensions}{%
  \typeout{The font encoding is \f@encoding}                  %
  \typeout{The font family is \f@family}                      %
  \typeout{The font series is \f@series}                      %
  \typeout{The font shape is \f@shape}                        %
  \typeout{The font size is \f@size}                          %
  \typeout{The baselineskip is \f@baselineskip}               %
  \typeout{The math font size is \tf@size}                    %
  \typeout{The math script size is \sf@size}                  %
  \typeout{The math scriptscript size is \ssf@size}           %
  \typeout{The linewidth is \the\linewidth}                   %
  \typeout{The textwidth is \the\textwidth}                   %
  \typeout{The slant is \the\fontdimen1\font}                 %
  \typeout{The inter word space is \the\fontdimen2\font}      %
  \typeout{The inter word stretch is \the\fontdimen3\font}    %
  \typeout{The inter word shrink is \the\fontdimen4\font}     %
  \typeout{The extra space is \the\fontdimen7\font}           %
  \typeout{The xspace skip is \the\xspaceskip}                %
  \typeout{The hyphenation character is \the\hyphenchar\font} %
}
%% This is a simpler version of amsmath's 'sideset' command, which
%% allows prefixed sub- and superscripts.  Use as something like:
%%   $\prefixscripts{^{-2}}{Y}$
\newcommand{\prefixscripts}[2]{%
  \@mathmeasure\z@\displaystyle{#2}%
  \global\setbox\@ne\vbox to\ht\z@{}\dp\@ne\dp\z@
  \setbox\tw@\box\@ne
  \@mathmeasure4\displaystyle{\copy\tw@#1}%
  \@mathmeasure6\displaystyle{#2}%
  \dimen@-\wd6 \advance\dimen@\wd4 \advance\dimen@\wd\z@
  \hbox to\dimen@{}{\kern-\dimen@\box4\box6}%
}
%% When a symbol using \prefixscripts also has postfixed sub- and
%% superscripts, the postfixed scripts are set relatively high or low,
%% compared to the prefixed scripts.  This command improves that.  Use
%% as something like:
%%   $\scripts{^{-2}}{Y}{_{lm}}$
\newcommand{\scripts}[3]{%
  \@mathmeasure\z@\displaystyle{#2}%
  \global\setbox\@ne\vbox to\ht\z@{}\dp\@ne\dp\z@
  \setbox\tw@\box\@ne
  \@mathmeasure4\displaystyle{\copy\tw@#1}%
  \@mathmeasure6\displaystyle{#2#3}%
  \dimen@-\wd6 \advance\dimen@\wd4 \advance\dimen@\wd\z@
  \hbox to\dimen@{}{\kern-\dimen@\box4\box6}%
}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% My extension of the braket package for inner products        %%
%% This allows code like $\InnerProduct{s|h}$, which works much %%
%% like $\Braket{x|y}$.                                         %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{braket}
\makeatletter
% Use MnSymbol symbols without the package
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
% Now construct \Bbrakket and \InnerProduct commands
\let\protect\relax
\def\bbra#1{\mathinner{\llangle{#1}|}}
\def\kket#1{\mathinner{|{#1}\rrangle}}
\def\bbrakket#1{\mathinner{\llangle{#1}\rrangle}}
\def\Bbra#1{\left\llangle#1\right|}
\def\Kket#1{\left|#1\right\rrangle}
{\catcode`\|=\active
  \xdef\InnerProduct{\protect\expandafter\noexpand\csname InnerProduct \endcsname}
  \expandafter\gdef\csname InnerProduct \endcsname#1{%
    \begingroup
    \ifx\SavedDoubleVert\relax
    \let\SavedDoubleVert\|\let\|\IpDoubleVert
    \fi
    \mathcode`\|32768\let|\IPVert
    \left({#1}\right)
    \endgroup
  }
  \xdef\Bbrakket{\protect\expandafter\noexpand\csname Bbrakket \endcsname}
  \expandafter\gdef\csname Bbrakket \endcsname#1{\begingroup
     \ifx\SavedDoubleVert\relax
       \let\SavedDoubleVert\|\let\|\BbraDoubleVert
     \fi
     \mathcode`\|32768\let|\BraVert
     \left\llangle{#1}\right\rrangle\endgroup}
}
\def\IPVert{\@ifnextchar|{\|\@gobble}% turn || into \|
     {\egroup\,\mid@vertical\,\bgroup}}
\def\IPDoubleVert{\egroup\,\mid@dblvertical\,\bgroup}
\let\SavedDoubleVert\relax
\def\midvert{\egroup\mid\bgroup}
\def\SetVert{\@ifnextchar|{\|\@gobble}% turn || into \|
    {\egroup\;\mid@vertical\;\bgroup}}
\def\SetDoubleVert{\egroup\;\mid@dblvertical\;\bgroup}
\def\mid@vertical{\mskip1mu\vrule\mskip1mu}
\def\mid@dblvertical{\mskip1mu\vrule\mskip2.5mu\vrule\mskip1mu}
\makeatother
\newcommand{\Overlap}{\Braket}
\newcommand{\Mismatch}{\ensuremath{\text{MM}}}
\newcommand{\MM}[2]{\ensuremath{\Mismatch\left(#1,#2\right)}}
\newcommand{\TargetMismatch}{\ensuremath{\Mismatch_{\text{target}}}}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> Preamble.tex <==
%auto-ignore

\makeatletter

%% Smaller space between section number and name
\def\@seccntformat#1{\csname the#1\endcsname.~}%

%% Smaller space between preceding text and new section headings
\def\section{%
  \@startsection {section}
  {1} {\z@} {0.55cm \@plus1ex \@minus .02ex}%
    {0.225cm} { \normalfont\bfseries \centering}%
}%
\def\subsection{%
  \@startsection {subsection}
  {2} {\z@ } {0.45cm \@plus 0.8ex \@minus 0.2ex}%
  {0.1125cm}{\normalfont \bfseries \centering }}
\def\subsubsection{%
  \@startsection {subsubsection}
  {3} {\z@ } {0.4cm \@plus 0.6ex \@minus 0.1ex}%
  {0.075cm}{\normalfont \it \centering }}

%% Headers and footers
\newcommand{\surnames}[1]{\def\@surnamelist{#1}\relax}
\surnames{\ }
\ifx \@shorttitle \@empty
  % \def\@oddhead{\small \MakeUppercase{\@title} \hfill}
  % Do nothing
\else
  \def\@oddhead{\small \MakeUppercase{\@shorttitle} \hfill}
\fi
\ifx \@surnamelist \@empty
  % Do nothing
\else
  \def\@evenhead{\small \MakeUppercase{\@surnamelist} \hfill}
\fi
\def\@oddfoot{\reset@font\hfil\thepage\hfil}%
\def\@evenfoot{\reset@font\hfil\thepage\hfil}%
\g@addto@macro\maketitle{\global\@specialpagetrue\gdef\@specialstyle{plain}}

%% Less hyphenation
\hyphenpenalty=1000  % Default: 50
%\tolerance=9000      % Default: 9999

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package and nice colors

%% The following conflicts with \texorpdfstring in section headers
% %% First, patch a bug from revtex4 to allow use of \nameref
% \usepackage{xpatch}% http://ctan.org/pkg/xpatch
% \makeatletter
% \xpatchcmd{\@ssect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>*
% \xpatchcmd{\@sect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>
% \makeatother

\usepackage[colorlinks, plainpages=false,
hyperfigures=true]{hyperref}
% \usepackage[pagebackref=true, colorlinks, plainpages=false,
% hyperfigures=true]{hyperref}
% \renewcommand*{\backref}[1]{}
% \renewcommand*{\backrefalt}[4]{%
%   \ifcase #1 \or (Cited on p.~#2.) \else %
%   (Cited on pp.~#2.) \fi %
% }
\hypersetup{linkcolor=LinkColor}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=UrlColor}
\hypersetup{setpagesize=false}
% \hypersetup{unicode} % Clashes with '\G' command defined in Macros
\hypersetup{pdfborder=0 0 0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatother

%\numberwithin{equation}{section}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> UsePackages.tex <==
%auto-ignore

%% Basic font packages
\newcommand{\hmmax}{0}
\newcommand{\bmmax}{0}
\usepackage[T3,T1]{fontenc}
%\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it} % For \mathpzc fonts
\usepackage{mathrsfs} % For \mathscr fonts
\usepackage{bm} % For \bm fonts
\makeatletter
\@ifclassloaded{beamer}
  { % if this is a beamer document, use sans-serif fonts
    \typeout{UsePackages: Detected beamer}
    \usepackage{tgheros}
    \renewcommand*\familydefault{\sfdefault}
  }
  { % otherwise:
    \typeout{UsePackages: Did not detect beamer}
    \ifx\asybeamer\undefined % use times for articles
    \typeout{UsePackages: Detected article}
    \usepackage[varg]{txfonts} % For math
    \usepackage{tgtermes} % For text
    \else % use beamer fonts for asy documents with beamer
    \typeout{Fonts: Detected asy for beamer}
    \usepackage{tgheros}
    \renewcommand*\familydefault{\sfdefault}
    \fi
  }
\usepackage{microtype} % For nicer alignment of text
\def\MT@register@subst@font{
  \MT@exp@one@n\MT@in@clist\font@name\MT@font@list
  \ifMT@inlist@\else\xdef\MT@font@list{\MT@font@list\font@name,}\fi}
\makeatother

% %% Compact the text (smaller intra-word spacing)
% \AtBeginDocument{
%   \setlength{\spaceskip}
%   {0.875\fontdimen2\font
%     plus 0.925\fontdimen3\font
%     minus 1\fontdimen4\font}
% }

%% Spread out the text lines slightly
\linespread{1.0425}

%% No extra space after periods
%\frenchspacing

%% A few necessary packages
\usepackage{graphicx} %
\usepackage[x11names,svgnames,rgb]{xcolor} %
% \usepackage[all]{onlyamsmath} % Error on bad non-ams math
\usepackage{xspace}
%% And a few optional ones
\usepackage{braket}
\usepackage{accents}
%\usepackage{rotating} % 'sidewaystable' support
\usepackage{siunitx}
\usepackage{mathtools}
\DeclareSymbolFontAlphabet{\mathrm}{operators}

%% Define a few colors
\definecolor{CiteColor}{rgb}{0.18039, 0.18824, 0.57255}
%\definecolor{CiteColor}{rgb}{0.250, 0.250, 0.800}
\definecolor{UrlColor} {rgb}{0.741, 0.173, 0.000}
\definecolor{DarkUrlColor} {rgb}{0.500, 0.110, 0.000}
\definecolor{LinkColor}{rgb}{0.25098, 0.47843, 0.04706}
%\definecolor{LinkColor}{rgb}{0.000, 0.502, 0.118}


%% To get the current font parameters and linewidth in a LaTeX
%% document, put \ShowFont at the appropriate place.  The results will
%% be printed in the log file (and/or to screen).
\makeatletter %
\newcommand{\ShowFont}{%
  \typeout{The main font is \f@encoding \space \f@family \space %
    \f@series \space \f@shape \space at \f@size pt.}%
  \typeout{The math font sizes are \tf@size pt (main), \sf@size pt %
    (script), and \ssf@size pt (scriptscript).}%
  \typeout{The linewidth is \the\linewidth}} %
\makeatother %
%% See the LaTeX2e font selection guide for more details.
%% Note also that captions in revtex4 are typeset with \small; when
%%   most of the document is 10pt, \small is 9pt.
%% In beamer, the default font is cmss and the math font size 10.95pt.
%% In revtex4, we have the following widths:
%%            onecolumn   twocolumn
%%     10pt     510pt       246pt
%%     12pt     468pt       229pt
%% PRD editors resize things to fit in a 200x200pt box by default, but
%%   I like to keep figures bigger.


\usepackage{xargs}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

